Imagine a dragon made of seaweed: How images enhance learning in Wikipedia

Though images are ubiquitous across Wikipedia, it is not obvious that the image choices optimally support learning. When well selected, images can enhance learning by dual coding, complementing, or supporting articles. When chosen poorly, images can mislead, distract, and confuse. We developed a large dataset containing 470 questions & answers to 94 Wikipedia articles with images on a wide range of topics. Through an online experiment (n=704), we determined whether the images displayed alongside the text of the article are effective in helping readers understand and learn. For certain tasks, such as learning to identify targets visually (e.g., "which of these pictures is a gujia?"), article images significantly improve accuracy. Images did not significantly improve general knowledge questions (e.g., "where are gujia from?"). Most interestingly, only some images helped with visual knowledge questions (e.g., "what shape is a gujia?"). Using our findings, we reflect on the implications for editors and tools to support image selection.

==> OLD_discussion.tex <==
\section{Discussion}
In this paper, we tested for the first time the role of images in knowledge acquisition through Wikipedia trough an online user study. 

\subsection{Summary of Findings}
\textbf{Encyclopedic Images help visual recognition.}
We found that, in some cases, images enhance the ability of readers to learn, serving the \textbf{cognitive function} of supporting knowledge retention by providing extra non-textual information. Images are especially useful to retain ``visual'' knowledge, namely to visually recognize and distinguish the subjects of Wikipedia articles, and to record information about the physical characteristics of objects, especially when the image content is aligned to the information in the text. These findings suggest that images can be extremely useful in encyclopedic settings, since the ability to visually recognize and classify objects is a fundamental aspect of our behavior and everyday life \cite{bruce1994recognizing}. Unillustrated articles, while providing enough useful information to learn about generic aspects of a subject, do not offer a full visual description, hence affecting the ability of the reader to recognize objects. As a matter of fact, what determines accuracy in our image questions is not whether the participant read the article (image question scores are the same for baseline and experiment), but whether an image was present when the participants read the article. 

\textbf{Generic knowledge acquisition is not (always) supported by images.}
Unlike most literature around the role of illustrations in instructional settings (see Section \label{sec:related}), our results show that images are not necessarily  useful to retain generic information about the subject of an article. This might be due to the fact that the construction and content of both text and images on Wikipedia are inherently different than knowledge specifically built for education and learning. The nature of Wikipedia articles might be closer to generic web content, where images have not found to be useful for content retention \cite{beymer2007eye}, than to scientific papers and educational material where images/graphics have proven helpful for learning \cite{guo2020you,renkl2017studying}. Still, our qualitative analysis showed that images are helpful to answer generic questions related to style and epochs of visual arts and architecture subjects, suggesting that perhaps for some topics, images on Wikipedia help create that mental model of an object which is then used for inferences \cite{gyselinck1999role}.\mr{add something about scientific/historic illustrations as potential subjects to explore?}

 %\mr{harmony between text and images and the dual coding theory} 
%\mr{Limitation: image only: what about captions?}
%This has accessibility implications for users in under-resourced settings who may rely entirely on a textual description of the subject of an article rather than the accompanying image in absence of .

\subsection{Implications and Limitations}
Collectively, our findings shed a first light on the role of images for knowledge retention on Wikipedia. This work has several theoretical and practical implications.

\textbf{A framework for large-scale learning studies through Wikipedia.} To our knowledge, this work represents the first attempt to study the role of images in content acquisition through Wikipedia. We provide the first large opensource dataset to test reading comprehension through Wikipedia, as well as an end-to-end framework and a crowdsourcing-based setting to test how different designs and conditions impact knowledge acquisition via the online encyclopedia. Given the importance of Wikipedia on the web, and its key role as a learning platform, we hope that the analysis and data in this paper can offer a starting point for future quantitative research around online encyclopedic knowledge acquisition.
One limitation of our dataset is that our questions were manually generated by a small group of volunteers. While we asked annotators to follow a thorough process and take into account the interestingness of the questions for the general public, the pool of questions in our data might not reflect the actual information needs and interests of Wikipedia readers. Future research is needed to align our reading comprehension questions with readers' motivations, and to analyze how images are useful to satisfy the different information needs.
Moreover, while the dataset is the first of its kind, its scale can be further expanded by automating article, section, image, and question retrieval using Natural Language Processing to detect Wikipedia articles which include a physical description and automatically generate questions that can be verified in crowdsourcing settings. Another limitation of this data is its availability for English only. Expanding the dataset to other languages, and studying how images are used in knowledge acquisition by different language communities and cultures, is part of our future work. 

\textbf{Design Implications for Adding Images to Wikipedia.} 
Our findings show that images can be useful to support some aspects of learning. This further justifies and encourages the development of community-led efforts to add images to unillustrated Wikipedia articles, such as the \textit{Wikipedia Pages Wanting Photos \#WPWP} campaign\footnote{\url{https://meta.wikimedia.org/wiki/Wikipedia_Pages_Wanting_Photos_2022}}, or the \textit{Visible Wiki Women}\footnote{\url{https://whoseknowledge.org/initiatives/visiblewikiwomen/}} initiative. 
Furthermore, our in-depth analysis shows that the photographic quality of the image, as well as its relevance to the text, play a key role in knowledge acquisition. We found that images of low  quality can hinder the ability of participants to visually recognize the subject of the article, and that illustrated articles where the image content is aligned with the article text lead to better understanding of the object's visual characteristics (accuracy for visual questions is higher for higher visual consistency). This is in line with the first of the 10 recommendations for pictorial facilitation of text information  (the ``10 tenents for teachers'') from Carney and Levin \cite{carney2002pictorial}  ``Select pictures that overlap with text content''. 
While both image quality and consistency with text are covered as part of the suggestion for image insertions within Wikipedia's manual of style\footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Manual_of_Style/Images}}, these findings highlight the importance of these two aspects when it comes to foster knowledge acquisition. Future large-scale experiments could make use of automated analysis of visual content to determine what subjects, spatial arrangements, and image types are more useful to improve reading comprehension. Furthermore, existing multimodal machine learning frameworks that measure the alignment between images and text \cite{radford2021learning,srinivasan2021wit}, could be incorporated into image suggestion frameworks to select the best images for unillustrated articles, such as the \textit{add-an-image} task for newcomer editors\footnote{\url{https://www.mediawiki.org/wiki/Growth/Personalized_first_day/Structured_tasks/Add_an_image}}.
Alignment between images and their corresponding captions also plays an important role for text comprehension \cite{bernard1990using} and has a dedicated page in Wikipedia's manual of style \footnote{\url{https://en.wikipedia.org/wiki/Wikipedia:Manual_of_Style/Captions}}. While investigating the importance of captions in Wikipedia knowledge acquisition was outside the scope of this work, this is an area for future research which could be implemented with  the data and framework provided with this study.

%\item For Wikipedia Readers:  This has accessibility implications for visually-impaired users or others who may rely entirely on a textual description of the subject of an article rather than the accompanying image.

%\ea{There are distinctions between motivations in actual wiki use (citation?)--some can be trying to answer questions quickly for class, others are looking things up because they care. Use of multiple platforms is a + as the participants are motivated by different things. This has been observed in other studies with lab in the wild and prolific/turk. Worth exploring more in the future--interaction between images and motivation.}

%\item For Wikipdia Readers:  

% crowdsourcing image annotations, so that images could be shown on demand if someone is interested in specific aspects of an article



==> OLD_discussion2.tex <==
\section{Discussion and Conclusions}
\kr{Would be good if we can highlight which of our findings go beyond what Wikipedia already recommends for images (one of the reviewers commented that it seems all consistent with the existing guidelines)}

Wikipedia is enormously important in helping people learn about a variety of subjects. Images from Wikipedia are an integral part of this experience both on Wikipedia and where the content is repurposed (e.g., search engine result pages). Despite the many ``views'' Wikipedia images get every day, there is little knowledge of the role that images play in people's information uptake. We contribute an open-source curated question \& answer dataset to test knowledge comprehension and recall in Wikipedia. \added{Additionally,} our study \deleted{provides a view on this and make}\added{makes} several empirical contributions:

%\kr{did we find that images were harmful for any articles or question types? Or is the general conclusion that we should always add images and they may just not always help? }

\paragraph{Learning about general aspects is rarely supported by images.} \deleted{Unsurprisingly,} We found that images do not always help learning about general aspects of a topic---in fact, participants were as likely to correctly answer general questions when the Wikipedia article did not include an image as they were when there was an image. However, our experiment \replaced{revealed}{did show} specific cases where images \textit{did} support answering general questions (see Fig. \ref{fig:nonimagequesiton}(a)). For example, remembering when a building was built or a painting was created may be easier with an image if the viewer can make inferences based on how that building or painting looked. \deleted{For example,} If a viewer generally recalls the properties of a romantic painting, they may be able to accurately estimate when a painting was made (even without seeing the date in text). For some topics (and with some background knowledge), images on Wikipedia may help readers create a mental model of an object, which they can then use for inferences~\cite{gyselinck1999role}. Future work may more generally identify when such images help and why.

\paragraph{Learning about visual aspects is only supported by images if they are consistent with the text}
Interestingly, the presence of images did not significantly improve answer accuracy for visual questions, such as questions about materials, color, or size. In fact, having an image or not resulted in the same answer accuracy in our study, suggesting that images, in general, do not support visual learning. This is perhaps the most surprising result of our study as images are commonly assumed to aid engagement and learning. However, consistent with our results, prior work studying the role of images in online contexts has also found that they may not support content retention~\cite{beymer2007eye}. 

In our follow-up analysis, we found that images that are consistent with their visual questions are answered accurately significantly more often than images that are inconsistent with the question. \deleted{There are two implications of this finding: First,} Images seem to boost answer accuracy when they are closely aligned with the text. This is consistent with some of the prior work \kr{but not with all of the prior work?} (e.g.,  \cite{peeck1993increasing}) and also with the first of the 10 recommendations for pictorial facilitation of text information  (the ``10 tenents for teachers'') from Carney and Levin \cite{carney2002pictorial}:  ``Select pictures that overlap with text content''. \added{However, in our visual consistency annotations, we found that less than 40\% of the image-visual question pairs in our dataset are aligned.} \replaced{Second, our finding}{Since visual questions are directly extracted from the article text, this} suggests that many images in Wikipedia  \replaced{are not optimally chosen to reflect the textual content in the article}{do not seem to be optimally chosen, perhaps because it is difficult for Wikipedia editors to anticipate what makes a good image}. .\kr{justify the claim (R3)} 

% A specific concern for future research is to identify those images that do not help, but may actively mislead or bias. For example, an image that only shows one representation of an entity may emphasize that form to the reader. This is particularly important as Wikipedia images are constantly being repurposed through automation in other contexts (e.g., search results). For example, the image for ``comfort food'' is a bowl of chicken soup. This Wikipedia-based image is displayed when searching for ``comfort food'' on Google. In the French Wikipedia, for topic (``Aliment-r\'econfort'') a sweet dessert is shown. However, the Google search for ``Aliment-r\'econfort'' shows the same chicken noodle soup as the English search. Awareness of how readers will engage with chosen images may impact how editors make their choices or Wikipedians define specific policies.

\paragraph{Images help visual recognition.}
We found that images generally enhance the ability of readers to visually recognize other instances of the object described in an article, compared to relying only on textual information. %This is especially the case when the image content is aligned with the information in the text. 
These findings suggest that images can be quite useful in encyclopedic settings, since the ability to visually recognize and classify objects is a fundamental aspect of everyday life \cite{bruce1994recognizing}. Unillustrated articles, while providing enough useful information to learn about general aspects of a subject, do not offer a full visual description. This may naturally affect the reader's ability to recognize objects of that class or instance. As a matter of fact, what determines accuracy in our image \added{recognition} questions is not whether the participant read the article (image \added{recognition} question scores are the same for \added{the} baseline and experiment \added{conditions}), but whether an image was present when the participants read the article. 


\paragraph{Photographic quality matters.} The cognitive theory of multimedia learning suggests that higher quality visuals reinforce and extend knowledge \cite{mayer2002multimedia}.  The results of our in-depth analysis align with this theory, showing that the photographic quality of the image plays a key role in knowledge acquisition from Wikipedia articles. We found that images of low  photographic quality (see, for example,  Figure~\ref{fig:imagequestion}(a)) can hinder participants' ability to visually recognize the subject of the article. Guidelines for image use in field guides, i.e., book used to recognize and research wildlife, indeed suggest that  high quality images are essential to make good educational material, especially when it comes to introductory sections and glossaries \cite{plantguide}. We also found that people may find it difficult to generalize  the insight from an image to other instances. For example, when shown an illustrated version of a plant, our participants were unable to accurately recognize the same plant in a photographed version. This could indicate that a dual representation is helpful, especially for article topics that are often sought out for learning what something looks like. \added{It also indicates that Wikipedia images are not always chosen to include representative features to be perceived as being of the same category, as the Prototype Theory suggests~\cite{}.}% that accurately crafted images in educational material make a good medium for the representational depiction of the way the world looks  \cite{tahririan2013analysis}.


%The finding also suggests that crowdsourcing image selection to  volunteers (Wikipedia editors) does come with the downside of a high variability in photographic quality. While the Wikipedia community has a significant amount of discussions on image selection~\cite{}, our findings indicate that partly obstructed objects should be replaced. 


 %\mr{harmony between text and images and the dual coding theory} 
%\mr{Limitation: image only: what about captions?}
%This has accessibility implications for users in under-resourced settings who may rely entirely on a textual description of the subject of an article rather than the accompanying image in absence of .

%\subsection{A Dataset for Image Q\&A}

\subsection{Design Implications}
Collectively, our findings have several theoretical and practical implications.

%%% describe for which articles images should always be available
\paragraph{Example images can support learning about historic eras} Our findings suggest that articles describing aspects about historical time periods, such as about specific paintings or architectural artifacts of a certain time, should include images. While architecture and visual arts figure among the top topics by image presence on Wikipedia \cite{gapsmap}, a large percentage of these articles still remain unillustrated. A concrete step building on our results could be to promote initiatives that encourage articles about such topics include high-quality images. \added{Moreover, existing editor groups who work on improving Wikimedia content on these topics, such as WikiProject Cultural Heritage on Wikidata \cite{wdculturalheritage}, or Wikiproject Historic Sites on Wikipedia \cite{wphistoricareas} , could explicitly encourage contributions to the visual content of the articles and items in these domains}.  

%\textbf{\kr{add cases where articles should definitely have an image?}}

\paragraph{Promote the addition of missing images on Wikipedia} 
Our findings show that images can be useful to support some aspects of learning. This further justifies and encourages the development of community-led efforts to add images to unillustrated Wikipedia articles, such as the \textit{Wikipedia Pages Wanting Photos \#WPWP} campaign \cite{WPWP}, or the \textit{Visible Wiki Women} \cite{visible} initiative, as well as those ``Wiki Loves'' campaigns designed to improve the visual coverage of encyclopedic topics, such as monuments (\textit{Wiki Loves Monuments} \cite{WLM}), or natural heritage (\textit{Wiki Loves Earth} \cite{WLE}).
.

\paragraph{Encourage or suggest images that are consistent with the text.} While Wikipedia editors can freely choose what images to add, our findings show that the chosen images are not always optimal. In fact, our analysis showed that images that are relevant to the text lead to higher accuracy in answering visual questions. Wikipedia's manual of style \cite{manualofstyle} already suggests to choose consistent images, but our dataset shows that this is not always followed. \added{While the manual of style speaks to the importance of image relevance to the generic ``topic's context'', we find here that images that are not aligned with the visual description of the subject can hinder the ability to learn.} Additional guidelines and examples may be needed for ensuring that images are consistent with descriptive text and to alert editors of the negative impact of inconsistent images.  Additionally, existing multimodal machine learning frameworks that measure the alignment between images and text \cite{radford2021learning,srinivasan2021wit}, could be incorporated into image suggestion frameworks to select the best images for unillustrated articles, such as the \textit{add-an-image} task for newcomer editors \cite{addimage}.

\paragraph{Discourage low-quality images.} Our study also reveals that images of low quality can hinder participants' ability to visually recognize the subject of the article.  The English Wikipedia manual of style \cite{manualofstyle} indeed suggests that images of ``Poor-quality images—dark or blurry; showing the subject too small, hidden in clutter, or ambiguous; and so on—should not be used unless absolutely necessary''. Automated image quality classifiers \cite{beytia2022visual} have been trained based on images labeled as ``Quality Images'' \cite{qualityimages} by the Wikimedia Commons community. To promote the usage of high quality images, similar computer vision-based classifiers could be incorporated into image suggestion algorithms, or search tools, that help editors find the right images for Wikipedia articles.  %While computer vision allows  \kr{is Wikipedia not automatically detecting this?}

\subsection{Broader Implications for Wikiwork}
%Improved tools may help editors add or replace images. This reduces the cost but does not necessarily increase the incentives for this kind of labor. 
Wikiwork---human contributions that improves Wikipedia in some way---is extremely varied. Some editors add new articles while others focus on improving citations or correcting grammar mistakes. Unfortunately, it is not obvious that image-focused wikiwork is as widely understood or appreciated.

We see a reflection of this in the Barnstars awarded by the Wikipedia community to editors~\cite{kriplean,barnstars}. Barnstars can be awarded for everything from diligence to being a `surreal contributor' (``any Wikipedian who adds `special flavor' to the community by acting as a sort of wildcard''). The range of these awards provide a partial signal of what kind of work is valued. While there are hundreds of types of Barnstars only a handful are dedicated to any kind of image work.
For example, an SVG Barnstar is awarded to those converting raster to vector images. A Valued Picture Barnstar is awarded to, ``users that uploaded a free image to Wikipedia that is considered wonderful, valuable, and/or crucial'' and the Photographer Barnstar goes to users ``who tirelessly improve Wikipedia with their photographic skills and contributions.''~\cite{barnstars}. %Even these limited accolades seem to be awarded rarely. For example, a search in September of 2022 shows no more than 2000 editors having a Photographer Barnstar in the English Wikipedia, compared  %Commons Ambassador Barnstar goes to, ``users who make exceptional contributions to the synergistic relationship of English Wikipedia with Wikimedia Commons by searching through Commons to find suitable pictures to add to English Wikipedia or finding free-use images on English Wikipedia and moving them to Commons''~\cite{barnstars}. Even these limited accolades seem to be awarded rarely. For example, a search in September of 2022 shows no more than 200 editors having a Commons Ambassador Barnstar in the English Wikipedia.

%Just as good wikiwork behaviors are rarely rewarded when it comes to images, bad behaviors are not always sanctioned or reversed. For example, placing images in articles does not require significant effort. 
 %specific instance of this may be an individual who copies the same image of a train--pos\citsibly one they took---to 
The findings in our paper also highlight the importance of adding high-quality images to Wikidata. Wikidata is a Wikimedia project and the open, manually curated knowledge graph that allows one to connect all Wikipedia articles across different languages. For example, the Train article exists in 162 languages, that often inherit structured information and the infobox image from the corresponding Wikidata item \cite{wikdiatatrain}, either manually or automatically.  %Additionally, an individual may copy the same image of a train to  (a real example from~\cite{he2018the_tower_of_babel}). 
Such an image may not be `best' or even `good' and certainly may not be culturally appropriate. While highly edited languages may counteract this kind of behavior and replace the image, languages with lower editorial resources may not. 

Our work demonstrates the importance of good images for a variety of learning objectives. As learning represents a key use case for Wikipedia~\cite{singer2017we}, wikiwork focused on curating, finding, or creating good images should be more valued. Although Barnstars alone are unlikely to provide motivation on their own, acknowledging work is a key component in increasing editor retention and norm-setting~\cite{matiasvolunteers}. Exactly what this kind of image-focused contribution looks like, and what types should be prioritized, is the topic of future work. Given resource limitations on good fair-use images, creating images may be crucial. Selecting culturally appropriate images for different Wiki language domains may also be an important form of labor. 

In addition to `novel' types of wikiwork, image-centered contributions can also become integrated into existing structures. For example, editors within a subtopic (e.g., birds, sociology, food, etc.) will often agree on templates and structures for those pages around text or infoboxes. Such constraints are difficult for images. For example, we may want all bird pages to have a consistent look and feel for their images, but the perfect image may not exist (or may not be in fair-use). While subject-matter experts disagree over whether photographs or paintings/illustrations are best for characterizing the world~\cite{birdguide,plantguide}, there is general agreement that a consistent look is important.
This presents a unique and interesting sociotechnical challenge.

The best interventions to normalize and prioritize image-centered wikiwork, all within the unique `bureaucracy' of Wikipedia~\cite{butler2008don}, present important future topics for research. 

%\item For Wikipedia Readers:  This has accessibility implications for visually-impaired users or others who may rely entirely on a textual description of the subject of an article rather than the accompanying image.

%\ea{There are distinctions between motivations in actual wiki use (citation?)--some can be trying to answer questions quickly for class, others are looking things up because they care. Use of multiple platforms is a + as the participants are motivated by different things. This has been observed in other studies with lab in the wild and prolific/turk. Worth exploring more in the future--interaction between images and motivation.}

%\item For Wikipdia Readers:  

% crowdsourcing image annotations, so that images could be shown on demand if someone is interested in specific aspects of an article

\subsection{Limitations and Future Work}
We hope that our manually curated question \& answer dataset to test knowledge comprehension in Wikipedia can be used and extended for other studies of images on Wikipedia. For example, our current dataset is focused on showing one specific image alongside the text (the so-called `lead' image). However, there is no evidence that this is the best image of a concept that Wikipedia or the Commons has to offer. A natural extension would be to experimentally vary the image displayed alongside the text with others that are available in the Commons. Such a use would provide guidance for editors, and potentially tool builders, in identifying not just a reasonable image, but the best one among a set.

A limitation of our dataset is that our questions were manually generated by a small group of researchers. Although we asked the annotators to follow a thorough process and take into account the interestingness of the questions for the general public, the pool of questions in our data might not reflect the actual information needs and interests of Wikipedia readers. Future research is needed to align our reading comprehension questions with readers' motivations, and to analyze how images are useful to satisfy the different information needs.

Moreover, while the dataset is the first of its kind, its scale can be further expanded by automating article, section, image, and question retrieval using Natural Language Processing to detect Wikipedia articles which include a physical description and automatically generate questions that can be verified in crowdsourcing settings.  %Moreover, expanding the dataset to other languages, and studying how images are used in knowledge acquisition by different language communities and cultures, is part of our future work. 
Such larger datasets would enable larger-scale experiments, which could make use of automated analysis of visual content to determine which subjects, spatial arrangements, and image types are more useful to improve reading comprehension.

Alignment between images and their corresponding captions also plays an important role for text comprehension \cite{bernard1990using}. This topic even has a dedicated page in Wikipedia's manual of style \cite{manualofstyle}. While investigating the importance of captions in Wikipedia knowledge acquisition was outside the scope of this work, this is an area for future research which could be implemented with the data and framework provided with this study.

Our study is also limited by being offered only in English. Our findings may not generalize to other languages and people from other countries and cultures. Future work could extend our study to a more diverse population to study the helpfulness of images with a sample more representative of Wikipedia users. 

In this initial work, we have focused on both a set of assumed motivations and learning objectives for reading Wikipedia. While we believe our choices are a good proxy for common tasks on Wikipedia, they do not represent the full breadth and complexity of the space. Additional research, with more types of images, articles, levels of expertise, learning objectives, assessments, and so on, will further clarify which images are contextually useful.



==> figures/results_qualitative/qualitative-results1.tex <==
\begin{figure*}
    \centering
    \captionsetup{justification=centering,margin=4mm}
    \begin{subfigure}[t]{0.6\textwidth}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/Irelands_history.jpg}
        \caption*{\footnotesize \\During which period was Newgrange built?\\}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/320px-Wwp50roof.jpeg}
        \caption*{\footnotesize When was the Worldwide Plaza completed?}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/Leonardo_da_vinci_-_La_scapigliata.jpg}
        \caption*{\footnotesize \\When was "La Scapigliata" painted?}
    \end{subfigure}
    \caption{General knowledge questions where images help with content retention.}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[t]{0.4\textwidth}
    \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/WHAT_MATERIALFlorence_-_David_by_Donatello.jpg}
        \caption*{\footnotesize \\What is the material of Donatello’s David?}
    \end{subfigure}
    \begin{subfigure}[t]{0.47\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/HOW_TALL_320px-Two_Brothers_totem_pole_Jasper.jpg}
        \caption*{\footnotesize \\How tall can totem poles be?}
    \end{subfigure}
    \caption{Visual knowledge questions where images help content retention.}
    \end{subfigure}
    \captionsetup{justification=justified}
    \caption{Qualitative analysis--examples of images that are helpful to answer generic questions. (a) Visual arts characteristics for general knowledge questions. (b) Visually consistent images for visual knowledge questions.}
    \label{fig:nonimagequesiton}
\end{figure*}



==> figures/results_qualitative/qualitative-results2.tex <==
\begin{figure*}
\centering
\captionsetup{justification=centering}
    \begin{subfigure}[b]{0.32\textwidth}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/LOWQ-320px-Spectral_bat_photo.jpg}
        \caption*{\footnotesize Low quality  (\textit{Spectral Bat})}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/HIGHQ320px-Leafy_Seadragon_on_Kangaroo_Island.jpg}
        \caption*{\footnotesize High quality  (\textit{Leafy Seadragon})}
    \end{subfigure}
    \caption{Image quality}
    \end{subfigure}\hfill
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.32\textwidth}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/PART-320px-2005-09-20_1080x1920_chicago_900_north_michigan.jpg}
        \caption*{\footnotesize Part (\textit{900 North Michigan})}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/WHOLE-800px-Chicago_900_North_Michigan_Avenue_(27940356553).jpg}
        \caption*{\footnotesize Whole (\textit{900 North Michigan})}
    \end{subfigure}
    \caption{Part VS Whole}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\textwidth}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/ILLUSTRATION-Calamintha_nepeta_Sturm54.jpg}
        \caption*{\footnotesize Illustrated\\ version (\textit{Nepeta})}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/results_qualitative/PHOTO-320px-Catnip-blossom.jpg}
        \caption*{\footnotesize Photographed version (\textit{Nepeta})}
    \end{subfigure}
    \caption{Photo VS Illustration}
    \end{subfigure}
    \captionsetup{justification=justified}
    \caption{In-depth analysis - examples of images that are harmful to answer the image question. (a) Low Quality images. (b) Images that describe only a part of the object. (c) Photographed objects in the article vs illustrations in the question.}
    \label{fig:imagequestion}
\end{figure*}


